Integrated Hardware Architecture and Device Placement Search

Distributed execution of deep learning training involves a dynamic interplay between hardware accelerator architecture and device placement strategy. This is the first work to explore the co-optimization of determining the optimal architecture and device placement strategy through novel algorithms, improving the balance of computational resources, memory usage, and data distribution. Our architecture search leverages tensor and vector units, determining their quantity and dimensionality, and on-chip and off-chip memory configurations. It also determines the microbatch size and decides whether to recompute or stash activations, balancing the memory footprint of training and storage size. For each explored architecture configuration, we use an Integer Linear Program (ILP) to find the optimal schedule for executing operators on the accelerator. The ILP results then integrate with a dynamic programming solution to identify the most effective device placement strategy, combining data, pipeline, and tensor model parallelism across multiple accelerators. Our approach achieves higher throughput on large language models compared to the state-of-the-art TPUv4 and the Spotlight accelerator search framework. The entire source code of PHAZE is available at https://github.com/msr-fiddle/phaze.

==> body/algorithms/pruner.tex <==
\begin{algorithm}
\caption{Heuristics to generate architectural configurations to explore.}
\label{alg:config_gen}

\newcommand{\funccommd}[1]{{\scriptsize\textcolor{DarkOrchid}{#1}}}
\newcommand{\mycommfont}[1]{{\scriptsize\itshape\textcolor{OliveGreen}{#1}}}

\scriptsize

\begin{algorithmic}
\STATE\textbf{Input} {$H\_level$ \quad \quad \quad \quad \quad \quad \quad \quad \quad $\mycommfont{// Hysteresis~ Level}$}
\STATE\textbf{Input} {$acc\_configs\_sorted$ \quad \quad \quad $\mycommfont{// Accelerator~ configurations~ sorted~ by~ area}$}

%\DontPrintSemicolon


\WHILE{$not~converged$}

    \STATE $curr\_area = curr\_config.area$

    \STATE $curr\_avg\_t = \funccommd{sum}(throughput ~ in ~ explored\_acc\_configs)$
    \STATE $max\_thpt\_per\_area[curr\_area] = \funccommd{max}(
            max\_thpt\_per\_area[curr\_area], curr\_avg\_t)$

    \IF {$\funccommd{all\_configs\_in\_area\_explored}$($curr\_area$)}
    
        \STATE $next\_area = acc\_sorted[curr\_area\_idx + 1]$

        \STATE $larger\_area\_thgpt = [max\_thpt\_per\_area[area]$
                                 for area in $acc\_sorted$]

        \IF { $\funccommd{len}($larger\_area\_thgpt)$ < H\_level$}
        
            \STATE \textbf{\textcolor{Blue}{return}} $next(config\_iter)$
        
        \ELSE
            \STATE $larger\_area\_thgpt = larger\_area\_thgpt[-H\_level:]$
            
            \STATE $converged = \funccommd{check\_if\_decreasing\_order}(larger\_area\_thgpt)$

           \STATE\textbf{\textcolor{Blue}{return}} $converged, next(config\_iter)$
        \ENDIF
        
    \ELSE
        \STATE \textbf{\textcolor{Blue}{return}} $False, next(config\_iter)$
    
\ENDIF
    

\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> body/limitations.tex <==
\section{Limitations}

%In designing \phaze, we make the following assumptions:

\niparagraph{Network topology and bandwidth.}
%
We assume a homogeneous network where all devices communicate with each other. Hierarchical or multi-level network topologies are not considered within the scope of this work. This assumption extends to collective operations across both tensor model parallel and data parallel frameworks.

\if 0
\niparagraph{Assumptions for scheduling operators in a layer on the accelerator using ILP.} 
%
We assume that the accelerator's global buffer can support parallel operator execution across cores (only when operators are not executing in intra-operator parallel).
%
Thus our assumption is only optimistic when the branching in the graph is very high. 
%
However, we empirically observe that ILP often selects intra-operator parallel mode for larger operators, wherein the global buffer utilizes a pipelined strategy to feed cores.


\niparagraph{Scheduling layers in a single stage of pipeline.}
%
Our dynamic programming algorithm operates under the assumption of serial execution when scheduling multiple layers within a single pipeline stage. While this hypothesis aligns with the sequential nature of current language models' layers, the ideal scenario would incorporate a layer scheduling algorithm.
%
\fi 

\niparagraph{Uniform tensor model parallel assumption.}
%
For tensor model parallelism, for every supported TMP width $t$,
we assume that every layer in the model that can be split is split ($t$-wise).
This is the style of TMP used in Megatron.


==> body/tables/stashingvsrecompute.tex <==
\begin{scriptsize}
\newcommand\ExtraSep
{\dimexpr\cmidrulewidth+\aboverulesep+\belowrulesep\relax}

\newcolumntype{?}{!{\vrule width 2pt}}
\setlength\extrarowheight{3pt}

\begin{table}
\centering
\caption{Architecture configuration and Device Placement strategy with activation stashing and without activation recomputation. Only models, which only were able to execute in both the modes are provided here. Other models only executed in activation recomputation. Table also provides the \% of throughput when activation recomputation is employed, instead of stashing.}
\resizebox{1\columnwidth}{!} 
{\begin{tabular}{ l | c | c | c | c | c }
 \hline 
\textbf{Model} & \multicolumn{2}{c}{\textbf{Architecture Configuration}}& \multicolumn{2}{c}{\textbf{Device Placement Strategy}}  & \textbf{\% of} 
\\
 & \textbf{With Recomputation} & \textbf{With Stashing} & \textbf{With Recomputation} & \textbf{With Stashing} & \textbf{Throughput} \\
 \hline
BertLarge~\cite{bert} &  &  &  &  & 
 \\
\hline
\multicolumn{6}{l}{\textbf{Tensor Model Parallel Models}} \\
\hline
BertLarge~\cite{bert} &  & & & & $XX$
 \\
MegatronGPT2-XL~\cite{shoeybi2020megatronlm}   &  &  &  &  & $XX$
 \\
MegatronGPT2-72~\cite{shoeybi2020megatronlm}   & \{256, 64, 4, 64, 4\} & \{256, 64, 4, 64, 4\} & \{7, 18, 8\}  &  \{7, 18, 8\} &  &

\end{tabular}}

\label{tab:workloads}
\end{table}
\end{scriptsize}
